Physics-guided Design and Learning of Neural Networks for Predicting Drag Force on Particle Suspensions in Moving Fluids

Physics-based simulations are often used to model and understand complex physical systems and processes in domains like fluid dynamics. Such simulations, although used frequently, have many limitations which could arise either due to the inability to accurately model a physical process owing to incomplete knowledge about certain facets of the process or due to the underlying process being too complex to accurately encode into a simulation model. In such situations, it is often useful to rely on machine learning methods to fill in the gap by learning a model of the complex physical process directly from simulation data. However, as data generation through simulations is costly, we need to develop models, being cognizant of data paucity issues. In such scenarios it is often helpful if the rich physical knowledge of the application domain is incorporated in the architectural design of machine learning models. Further, we can also use information from physics-based simulations to guide the learning process using aggregate supervision to favorably constrain the learning process. In this paper, we propose PhyDNN, a deep learning model using physics-guided structural priors and physics-guided aggregate supervision for modeling the drag forces acting on each particle in a Computational Fluid Dynamics-Discrete Element Method(CFD-DEM). We conduct extensive experiments in the context of drag force prediction and showcase the usefulness of including physics knowledge in our deep learning formulation both in the design and through learning process. Our proposed PhyDNN model has been compared to several state-of-the-art models and achieves a significant performance improvement of 8.46% on average across all baseline models. The source code has been made available and the dataset used is detailed in [1, 2].

==> sections/nikhil_notes.tex <==
\iffalse 
\subsection{Model Description}
\begin{itemize}
    \item DNN  : Feed-forward Neural Network Model.
    \item DNN+ : Feed-forward Neural Network Model with auxiliary prediction of pressure samples in single architecture.
    \item DNN-MT-S: Feed-forward Neural Network Model with separate models (with $S$ shared layers) one predicting drag force on the particle and the other predicting pressure samples. 
    \item DNN-All : Feed-forward Neural Network Model trained on all data but tested on specific test set.
    \item DNN-MT-Split-S: Feed-forward Neural Network Model with 4 separate models (with $S$ shared layers) one predicting drag force, the other predicting shear and pressure drag components (i.e Drag Force Split Into Its Component Parts) with the fourth model predicting pressure samples.
\end{itemize}

\subsection{Paper Feedback}
\subsubsection{Introduction}
\begin{enumerate}
    \item Choice of intermediate variables.
    \item Point 3 section 1, model architecture is designed so that we predict intermediate variables that are useful in predicting the target. Entire model design is physics based.
    \item We are also learning the multiple tasks differently 
    \item Statistical regularizer in section 1, point 4.
    \item Change weak supervision to something else like coarse-grained supervision etc. 
    \item This model is also taking a step towards explainability as the auxiliary tasks provide a look into the model.
\end{enumerate}

\subsubsection{Results}
\begin{enumerate}

    \item Show pressure,shear component weights. For this experiment, train on all data, during testing, disaggregate the results and plot errors per (RE,SF) pairs for both shear and pressure component. 
    \item Conduct experiment by training only on (low, high Re sets).
    
    \item Add Heat maps per RE,SF group.
    
    \item (Strict Generalizability during Extrapolation) Test generalizability by holding out high-(Re,Sf) and train only on low-(Re,Sf).
    
    \item (Generalizability during Interpolation) Test generalizability by holding out midrange-(Re,Sf) and train on low,high (Re,Sf)
    
    \item(Slightly Relaxed Generalizability) Test generalizability by holding out - (Re,Sf) and train only on low-(Re,Sf) but mask certain drag force targets out during training and only supply pressure, velocity fields.
    
    \item Show sensitivity of hyper-parameters for best performing model.
    
    \item Impact of training on different sizes of data.
    
    \item Can we still use TauY,PY,TauZ,PZ if there is some signal present within them?
    
    \item Instead of training all layers together, what if we pre-train first few layers and then train everything else. (layer-wise pre-training idea).
    Pre-train values by initializing hyper-parameter values of auxiliary tasks to high values initially and decreasing them.
\end{enumerate}

\subsubsection{Message}
\begin{enumerate}
    \item If we are solving a task, we want to think about what are the `auxiliary tasks` or `intermediate variables` that we want to think of that will help address the problem better.
    \item Architecture we have designed. (We need to use domain knowledge)
    \item Constraints we have added. 
    \item Add noise into main task and test.

\end{enumerate}


\subsubsection{Paper Writing}
\begin{enumerate}
    \item Results
    \item Problem Formulation (some portions that Dr. Tafti can help)
    \begin{enumerate}
        \item Motivation of problem.
        \item Why pressure, velocity field.
        \item Why pressure, shear component is important.
    \end{enumerate}
    \item Better ways to perform multi-task learning.
\end{enumerate}
\fi 

\subsection{ToDo}
\begin{enumerate}
    
    \item Line plot of how results vary with sparsity (run all \ourmethodAll results). (Nikhil) \nikhilc{(Done)}
    
    \item Sensitivity analysis for best performing model for 55\% training size (run with different hyper-parameters for pres,vel fields tasks and show how MSE,MRE change).
    Fix, pressure,vel. hyperparam to a particular value and use that value for all training fractions and see how much results change. (Nikhil) \nikhilc{(Done)}
    
    \item Aggregate analysis over all Re,Sf pairs for particular training fraction (55\%). We will show difference in performance of best baseline and our model. Each grid cell will be difference in performacne of error between our model and best baseline (look at DNN, CNN, DNN-MT-Pres., DNN-MT-Vel.). (Nikhil) \nikhilc{(Done)}
    
    \item Add pressure drag component to shear drag component predictions ratio per (Re,Sf) pair. Also compare this ratio to ground truth data. (Nikhil) \nikhilc{(Done)}
    
    \item Remove velocity field figures. (Nikhil) \nikhilc{(Done)}
    
    \item Change x-axis in pressure field plots. (Nikhil)
    
    \item Experimental Setup: (Nikhil)
    \begin{enumerate}
        \item Mention baseline descriptions.
        \item Mention descriptions of each evaluation metric.
        \item Make sure we mention all hyperparameters used for learning and model architecture.
    \end{enumerate}
    
    \item Compare best ablation model i.e model closest to PhyDNN models (DNN-MT-Pres., Dnn-MT-Vel.).
    
    \item Move all models (from notebooks) and create pipeline that will make it easy to run experiments. All models in NikhilModels/MultiTaskModels/ need to be converted into a pipeline. (Jie)
    
    \item Generalization experiment. (Jie)
        \begin{enumerate}
            \item Use 55\% training data and perform leave-one-out per (Re,Sf) combination.
            \begin{enumerate}
                \item Just run strong baselines (1 or 2) with PhyDNNAll , PhyDNN-PxTx.
            \end{enumerate}
            \item If this doesn't work, we can incorporate pressure and velocity fields into the training and just mask the drag force values.
        \end{enumerate}
        
    \item DNN with regularization. (Jie)
        \begin{enumerate}
            \item Try L2 norm.
            \item Try L1 norm.
            \item Try Dropout.
        \end{enumerate}
    
    \item We need a generic figure that talks about:  (Nikhil)
        \begin{enumerate}
            \item Physics Guided Architecture.
            \item Physics Guided Learning.
            \item Physics Guided Tasks.
        \end{enumerate}
        
    \item Move figure 1 to section 3.
\end{enumerate}

==> sections/results_and_discussion_old.tex <==
\iffalse 
\begin{figure}
\includegraphics[width=\linewidth]{figures/{{H = 50, 2 hidden layers (with Normalization)}.png}}
\caption{Training Performance at 2 Hidden Layers of Size 50}
\label{fig:H50h2N}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{figures/{{H = 50, 5 hidden layers (with Normalization)}.png}}
\caption{Training Performance at 5 Hidden Layers of Size 50}
\label{fig:H50h5N}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{figures/{{Test_simple_feed_forward}.png}}
\caption{Results on Test Set at Best Settings Using Simple Feed-forward Neural Network}
\label{fig:TestSimple}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{figures/{{Training_One_Hot}.png}}
\caption{Results on Training Set Using 3D One-hot Encoding ANN}
\label{fig:TrainingOnehot}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{figures/{{Test_One_Hot}.png}}
\caption{Results on Test Set Using 3D One-hot Encoding ANN}
\label{fig:TestOnehot}
\end{figure}
\fi 
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         Model & MSE  & MRE (\%)\\ \hline 
         DNN & 9.079 & 10.2 \\ \hline 
         DNN-En & 6.418 & \textbf{7.3} \\ \hline 
         CNN & \textbf{5.274} &7.6 \\ \hline
    \end{tabular}
    \caption{Performance Comparison. Models include simple feed-forward neural network (DNN), DNN with spatial one-hot encoding (DNN-En), standard convolutional neural networks (CNN).}
    \label{tab:my_label}
\end{table}

In the table~\ref{tab:my_label}, add results for Mean Squared Error and Mean Relative Error for the Deep Neural Network (DNN) and Conv. Neural Net (CNN) model that we have so far and inclue all other variants as additional rows in the same table.

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         Model & MSE  & MRE (\%)\\ \hline
         DNN    &9.903 & 24.9 \\ \hline
         DNN-MT & 7.297 & \textbf{21.8}\\ \hline
         DNN+ & \textbf{7.06} & 22.1 \\ \hline
    \end{tabular}
    \caption{Performance Comparison. DNN is the feed-forward neural network. DNN-MT is the feed-forward multi-task model wherein, in addition to the drag-force on a particle, the pressure field around the particle is predicted as an auxiliary task. DNN+ is the model wherein a common NN is used to predict both the sample pressure points around the particle as well as the drag force on the particle. All results are reported for \textbf{RE=50 \& SF = 0.2}. }
    \label{tab:my_label}
\end{table}
